Behind Maya: Building a Multilingual Vision Language Model

In recent times, we have seen a rapid development of large Vision-Language Models (VLMs). They have shown impressive results on academic benchmarks, primarily in widely spoken languages but lack performance on low-resource languages and varied cultural contexts. To address these limitations, we introduce Maya, an open-source Multilingual VLM. Our contributions are: 1) a multilingual image-text pretraining dataset in eight languages, based on the LLaVA pretraining dataset; and 2) a multilingual image-text model supporting these languages, enhancing cultural and linguistic comprehension in vision-language tasks. Code available at https://github.com/nahidalam/maya.

==> sec/2_relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}


%-------------------------------------------------------------------------
\subsection{Multilingual Large Language Models}

While open-source large language models have made notable strides, progress in multilingual LLMs (mLLMs) still lags. Many LLMs \cite{team2024gemma2, dubey2024llama, abdin2024phi, ministral} offer limited multilingual support, typically focusing on high-resource languages with reduced performance in others. Dedicated mLLMs \cite{xue2020mt5, lin2021few, le2023bloom, qwen, lin2024mala, ustun2024aya, aryabumi2024aya}, such as BLOOM \citep{le2023bloom} and Aya-101 \citep{ustun2024aya}, extend language coverage to 43 and 101 languages respectively, improving performance across tasks like translation, summarization, and reasoning.

%-------------------------------------------------------------------------
\subsection{Multimodal Large Language Models}

Research in Multimodal Large Language Models (MLLMs) has advanced significantly in enabling models to process both images and text across diverse tasks, with progress along two main paths: proprietary closed-source systems \cite{gpt4o, team2023gemini, claude} and open-source initiatives. While most of the initial efforts focused predominantly on English-language capabilities, such as LLaVA \cite {liu2023llava, liu2023improvedllava}, several recent works have attempted to close this gap by targeting non-English languages. PALO \cite{maaz2024palo} extended LLaVA \cite{liu2023llava} to cover 10 major languages via semi-automated translations of the LLaVA-Instruct-150k dataset \cite {liu2023llava}. X-LLaVA \cite{shin2024x} demonstrated strong Korean-English bilingual performance. Broader language coverage has been achieved by Llama 3.2 \cite{dubey2024llama} supporting 8 languages and Qwen2-VL \cite{wang2024qwen2} covering several European languages alongside Japanese, Korean, Arabic and Vietnamese. More recent developments have pushed multilingual boundaries through diverse approaches: PaliGemma \cite{beyer2024paligemma} pretrained on a variety of vision-language tasks upto 35 languages providing an open base MLLM but without instruction tuning, \cite{geigle2023mblip} mBLIP realigned English-tuned image encoder using machine-translated data for 95 languages, Pangea \cite{yue2024pangea} is a multilingual multimodal model trained on an instruction dataset spanning 39 languages, Parrot \cite{sun2024parrotmultilingualvisualinstruction} addressed supervised fine-tuning imbalances across 6 languages through textual guidance for visual token alignment, while models like Phi-3.5-Vision \cite{abdin2024phi}, Pixtral \cite{agrawal2024pixtral} and Molmo \cite{deitke2024molmo} are mostly English-centric \cite{yue2024pangea}.

%-------------------------------------------------------------------------
\subsection{Multimodal Multilingual Datasets}

Large-scale datasets for retrieval and captioning such as xFlickrCO \citep{bugliarello-etal-2022-iglue}, BLIP3-KALE \citep{awadalla2024blip3kaleknowledgeaugmentedlargescale} and WIT \citep{wit_2021} have been developed to support broader multimodal research. For instruction tuning, PALO \cite{maaz2024palo} built a dataset of 150K images in 10 languages from a subset of LLaVA image-text instruction tuning dataset on English text, while Pangea \cite{yue2024pangea} demonstrated broader coverage with image-text pair dataset in 39 languages.

%-------------------------------------------------------------------------
\subsection{Evaluating Multimodal Models}

Evaluating multilingual multimodal LLMs \cite{beyer2024paligemma, wang2024qwen2, yue2024pangea} involves two main categories. The first assesses standard multimodal tasks, such as cross-lingual visual question answering (VQA) with xGQA \citep{pfeiffer2021xgqa} and image-text retrieval via xFlickrCO \citep{bugliarello-etal-2022-iglue}. The second evaluates cultural understanding, using datasets like MaRVL \citep{liu-etal-2021-visually} for visual reasoning, CVQA \citep{romero2024cvqa} for cultural context, and XM3600 \citep{thapliyal2022crossmodal} for cross-modal comprehension. Significant progress has been made in developing multilingual multimodal datasets for evaluating VLMs including XVNLI \citep{bugliarello-etal-2022-iglue} for visual natural language inference, MTVQA \citep{tang2024mtvqa} for temporal reasoning, M3Exam \citep{zhang2023m3exam} for educational assessment, PangeaBench \cite{yue2024pangea} for broad multilingual capabilities, MMMB \cite{sun2024parrotmultilingualvisualinstruction} for cross-lingual understanding, and LLaVA-Bench-In-The-Wild \cite{liu2023llava, maaz2024palo} for real-world scenarios. Notably, none of these datasets focus on evaluating toxicity.

%-------------------------------------------------------------------------


==> sec/6_boarderimpact.tex <==
\section{Broader Impact}
\label{sec:broaderimpact}

Maya enables high-quality AI-driven content generation across linguistic and geographic boundaries by leveraging a diverse corpus of multilingual and multimodal data. This addresses a critical gap in AI capabilities, particularly for low-resource languages.

To ensure the ethical and safe deployment of Maya, we have implemented rigorous data curation processes to eliminate toxic and harmful content, such as hate speech, violence, and explicit material. While we have made every effort to remove such content, it is important to acknowledge that residual traces may still exist. To facilitate further research and development in this area, we will make the toxicity-free dataset and model weights publicly available to the research community. This will empower researchers and developers to build upon our work and advance the state-of-the-art in inclusive and responsible AI.

By prioritizing diversity, equity, and safety, Maya contributes to the creation of more inclusive and culturally sensitive AI systems, fostering respectful and meaningful interactions on a global scale.

==> sec/8_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
